BoSy: An Experimentation Framework for Bounded Synthesis

We present BoSy, a reactive synthesis tool based on the bounded synthesis approach. Bounded synthesis ensures the minimality of the synthesized implementation by incrementally increasing a bound on the size of the solutions it considers. For each bound, the existence of a solution is encoded as a logical constraint solving problem that is solved by an appropriate solver. BoSy constructs bounded synthesis encodings into SAT, QBF, DQBF, EPR, and SMT, and interfaces to solvers of the corresponding type. When supported by the solver, BoSy extracts solutions as circuits, which can, if desired, be verified with standard hardware model checkers. BoSy won the LTL synthesis track at SYNTCOMP 2016. In addition to its use as a synthesis tool, BoSy can also be used as an experimentation and performance evaluation framework for various types of satisfiability solvers.

==> bounded_synthesis.tex <==
\section{Bounded Synthesis}



==> implementation.tex <==
\section{Implementation}


The implementation is divided into a single \emph{frontend} that is responsible for parsing the input format and constructing the automaton representation, and multiple \emph{backends} that are responsible for creating and solving the generated constraint systems.
The backends differ in the expressiveness of the underlying logic, e.g. there is a pure propositional encoding which uses a SAT solver and other encodings that employ quantification and use QBF or first-order solver~\cite{encodings}.
The frontend and backend are connected by \emph{search strategies}.
They determine the initial bound and control the bound increments in case of unsatisfiable queries.
Currently, we have implemented a linear and an exponential search strategy.
By default, the implementation searches of a realizing strategy and a counterexample strategy in parallel.





\paragraph{Frontend.}
The component structure of the frontend is depicted in Fig.~\ref{fig:frontend}.
$\bosy$ accepts a JSON-based input format that contains the input and output signals, the target semantics, and a list of LTL formulas partitioned into assumptions and guarantees.
An example is shown in Fig.~\ref{fig:json_input}.

After parsing, the LTL formula is transformed into an equivalent universal co-B\"uchi automaton.
Currently, we support $\ltlthreeba$~\cite{conf/tacas/BabiakKRS12} and $\spot$~\cite{conf/atva/Duret-LutzLFMRX16} for this conversion, but further transformation tools can be integrated easily.
To the resulting automaton, we apply some basic optimization steps like replacing rejecting terminal states with safety conditions and an analysis of strongly connected components to reduce the annotation~\cite{journals/sttt/FinkbeinerS13}.

%%TODO mark plug and play in pictures
%\begin{figure}[t]
%  \centering
%  \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,thick,scale=1,transform shape]
%    \tikzstyle{state}=[rounded corners,rectangle split, rectangle split parts=2, inner sep=5pt, draw]
%    
%    \node[state] (spec) {Specification \nodepart{two} {\tiny JSON representation}};
%    \node[state,below right=-.1cm and 1.5cm of spec] (automaton_conversion) {Automaton Conversion \nodepart{two}  ltl3ba};
%	\node[state,above right=-.3cm and 1.5cm of spec] (automaton_conversion2) {Automaton Conversion \nodepart{two} spot};
%    \node[state,right=6.5cm of spec] (automata) {Automata \nodepart{two} {\tiny graph representation}};
%	
%	\node[right=3.25cm of spec] {\bf \vdots};
%    
%    \draw (spec.east) edge[->,dotted, bend left=15] node[pos=0.3] {LTL} (automaton_conversion.west)
%    	  (spec.east) edge[->,dotted, bend right=15] (automaton_conversion2.west)
%          (automaton_conversion.east) edge[->] node[below right] {SPIN never-claim} (automata)
%          (automata) edge[loop above] node {optimizations} ()
%          (automaton_conversion2.east) edge[->] node{HOA} (automata)
%          ;
%    
%  \end{tikzpicture}
%  \caption{Frontend Architecture (dotted lines represent experiment choices) }
%  \label{fig:frontend}
%\end{figure}

\paragraph{Backend.}
The role of a backend is to construct and solve a constraint system that is satisfiable if, and only if, there is a system with given size bound $n$ that satisfies the specification.
To enable synthesis, a backend should also be able to extract witnesses from satisfiable queries.
This extraction of the synthesized implementation, however, depends on the solver support.
Figure~\ref{fig:backend} gives a schematic overview over a backend that supports synthesis.

Given the specification automaton and a bound $n$, the backend constructs a constraint system using a logic representation which supports propositional logic, different kinds of quantification, and comparison operators (between natural numbers).
This constraint system is then translated to a format that the selected solver understands.
We have implemented the conversion from propositional constraints to the DIMACS file format used in SAT solvers, as well as the quantified extensions QDIMACS and DQDIMACS used in QBF and DQBF solvers.
Further formats include QCIR (QBF), TPTP3 (EPR) and SMT.
The witnesses extracted from satisfying queries, i.e., assignments from SAT solvers and Skolem functions from QBF solvers, are again translated into a functional representation of the synthesized implementation.

Our implementation contains the following backends.
We refer the reader to~\cite{encodings} for details.
\begin{itemize}
  \item A \emph{basic} propositional backend using a SAT solver.
  \item An \emph{input-symbolic} encoding using a QBF solver.
  \item Two encodings (\emph{state-symbolic},\emph{symbolic}) using DQBF/EPR solvers.
  \item An \emph{SMT} encoding resembling the original bounded synthesis encoding~\cite{journals/sttt/FinkbeinerS13}.
\end{itemize}

%\begin{figure}[t]
%  \centering
%  \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,thick,scale=1,transform shape]
%    \tikzstyle{state}=[rounded corners,rectangle split, rectangle split parts=2, inner sep=5pt, draw]
%    
%
%  
%    \coordinate (independent_start) at (-3.3,1);
%    \coordinate (independent_end) at (7,-1);
%    
%      \draw[rounded corners=4pt,fill=black!10] (independent_start) rectangle (independent_end);
%    \node[below right=0 and 0 of independent_start] {{\tiny solver-independent}};
%    
%    \coordinate (dependent_start) at (-3.3,-1);
%    \coordinate (dependent_end) at (7,-5);
%    \draw[rounded corners=4pt,fill=black!20] (dependent_start) rectangle (dependent_end);
%    \node[below right=0 and 0 of dependent_start] {{\tiny solver-dependent}};
%  
%    \node[state] (constraints) {Constraints \nodepart{two} {\tiny generic logic representation}};
%    %\node[state,below=of constraints] (solver_format) {Solver Format \nodepart{two} {\tiny (D)(Q)DIMACS, QCIR, TPTP3, SMT}};
%    
%    \node[state,right=1.5cm of constraints] (implementation) {Implementation \nodepart{two} {\tiny functional representation}};
%    \node[state,below=1.8cm of implementation] (certificate) {Certificate \nodepart{two} {\tiny assignments, functions}};
%    
%     \node[state, above=of constraints, dashed] (automata) {Automata \nodepart{two} {\tiny graph representation}};
%    
%	\node[state, above right=.3cm and 1.2cm of implementation, minimum width=2.2cm] (aiger) {Circuit \nodepart{two} AIGER};
%	\node[state, right=1.2cm of implementation, minimum width=2.2cm] (smv) {FSM \nodepart{two} SMV model};
%	\node[state, below right=.3cm and 1.2cm of implementation, minimum width=2.2cm] (dot) {Graph \nodepart{two} DOT};
%	
%	\node[state, below left=1cm and -.5cm of constraints] (sat) {SAT Solver\nodepart{two} {\scriptsize DIMACS}};
%	\node[state, right=1.6cm of sat] (smt) {SMT Solver\nodepart{two} {\scriptsize SMTLIB}};
%    \node[state, below right=.75cm and -2.05cm of sat] (qbf) {QBF Solver \nodepart{two} {\scriptsize QDIMACS, QCIR}};
%    \node[state, right=.4cm  of qbf] (dqbf) {DQBF / EPR \nodepart{two} {\scriptsize DQDIMACS, TPTP3}};
%    
%    \draw (automata) edge[->] (constraints)
%    	  (constraints.south) edge[dotted,->] (sat)
%    	  (constraints.south) edge[dotted,->] (qbf.45)
%    	  (constraints.south) edge[dotted,->] (dqbf.145)
%    	  (constraints.south) edge[dotted,->] (smt)
%          %(sat) edge[->] node {\scriptsize satisfiable} (certificate)
%          (certificate) edge[->] (implementation)
%          (constraints) edge[dashed,->] (implementation)
%          (implementation.east) edge[dotted,->] (aiger.west)
%          (implementation.east) edge[dotted,->] (smv.west)
%          (implementation.east) edge[dotted,->] (dot.west)
%          (sat.340) edge[->,bend right=5] (certificate.west)
%          (qbf.40) edge[bend left=5] (certificate.west)
%          (smt.340) edge[bend right=30] node[above right, pos=0.3] {\scriptsize sat} (certificate.west)
%          (dqbf.40) edge[bend left=20] (certificate.west)
%          ;
%    
%  \end{tikzpicture}
%  \caption{Backend Architecture (dotted lines represent experiment choices)}
%  \label{fig:backend}
%\end{figure}

\paragraph{QBF backend.}
The QBF backend takes a two-step approach for synthesis.
The bounded synthesis QBF query has the quantifier prefix $\exists \forall \exists$~\cite{encodings}.
In synthesis mode, the query is solved by a combination of QBF preprocessor $\bloqqer$~\cite{conf/cade/BiereLS11} and QBF solver $\rareqs$~\cite{journals/ai/JanotaKMC16}.
From a satisfiable query, the assignment of the top-level existential quantification is extracted~\cite{conf/date/SeidlK14} and then used to reduce the original query by eliminating the top level existential quantifier.
The resulting query, now with a $\forall \exists$ prefix, is then solved using a certifying QBF solver like $\quabs$~\cite{journals/corr/Tentrup16}, $\cadet$~\cite{conf/sat/RabeS16}, or $\caqe$~\cite{conf/fmcad/RabeT15}.
The resulting certificate is then translated into a functional representation of the synthesized implementation.

\paragraph{Output.}
Our representation of the synthesized implementation stores the transition function as $\tau: S \times S \rightarrow \bool(I)$ and the output functions as $f_o : S \times \bool(I)$ for every $o \in O$ where $S$ is the state space of the implementation, $I$ and $O$ are the input and output propositions, respectively.
From this representation, it is possible to translate the implementation into an AIGER circuit as required by the SYNTCOMP rules, to a SMV model, or to a graphical representation using the DOT format.
Examples are given in Fig.~\ref{fig:synthesized}

\subsection{Extensibility}

The following parts of the system are standardized and can be easily extended.

\paragraph{Backend.}
A backend has access to the automaton, the semantics, and the input and output signals.
It has to provide a method \texttt{solve} that has a bound as parameter and should return whether there is an implementation with the given bound that realizes the specification.
The method is implemented by building the constraint system and solving it using a theory solver.
One can either use our logic representation or build the textual solver representation directly.
If the backend supports synthesis, it implements a second method \texttt{extractSolution} that is called if \texttt{solve} returns true.
It returns a representation of the realizing implementation as described above.

\paragraph{LTL to automaton conversion.}
Tools that output $\spin$ neverclaims or the HOA format are supported.

\paragraph{Theory solvers.}
We support SAT solvers that accept the DIMACS input format and that can output satisfying assignments.
We have three categories of QBF solving tools: QDIMACS/QCIR solver that can output top-level assignments, QDIMACS preprocessors, and certifying QDIMACS/QCIR solver that can provide functions witnessing satisfiable queries.
For the remaining formats, i.e., DQDIMACS, TPTP3, and SMT, we only require format conformance as witness extraction is not supported, yet.

\paragraph{Targets.}
The provided encodings (AIGER, SMV, DOT) should give enough guidance to implement another target.

%\begin{itemize}
%  \item \emph{backends}: currently basic (SAT encoding), input-symbolic (QBF), state-symbolic, symbolic (both DQBF/EPR), and SMT (original encoding)
%  \item \emph{LTL to automaton}: currently $\ltlthreeba$ and $\spot$ using SPIN neverclaim format (HOA format in future)
%  \item \emph{solver}: DIMACS SAT solver that output assignments (currently $\picosat$ and $\cmsat$), QDIMACS/QCIR QBF solver that output top-level assignments (currently $\rareqs$ and $\depqbf$), QDIMACS preprocessors (currently $\bloqqer$), certifying QDIMACS/QCIR solver (currently $\quabs$), DQDIMACS solver (currently $\idq$), SMT solver (currently $\zthree$ and $\cvcfour$)
%  \item \emph{target}: currently AIGER as required by SYNTCOMP rules, SMV, and DOT
%\end{itemize}

